Estimating the HEVC Decoding Energy Using the Decoder Processing Time

This paper presents a method to accurately estimate the required decoding energy for a given HEVC software decoding solution. We show that the decoder's processing time as returned by common C++ and UNIX functions is a highly suitable parameter to obtain valid estimations for the actual decoding energy. We verify this hypothesis by performing an exhaustive measurement series using different decoder setups and video bit streams. Our findings can be used by developers and researchers in the search for new energy saving video compression algorithms.

==> gfx/power_time.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA Idle}%
\psfrag{012}[cl][cl]{\matlabtextA Decodingaa}%
\psfrag{013}[bc][bc]{\matlabtextA Power}%
\psfrag{014}[tc][tc]{\matlabtextA Time}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $30$}%
\psfrag{001}[ct][ct]{\matlabtextA $40$}%
\psfrag{002}[ct][ct]{\matlabtextA $50$}%
\psfrag{003}[ct][ct]{\matlabtextA $60$}%
\psfrag{004}[ct][ct]{\matlabtextA $70$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $2.2$}%
\psfrag{006}[rc][rc]{\matlabtextA $2.6$}%
\psfrag{007}[rc][rc]{\matlabtextA $3$}%
\psfrag{008}[rc][rc]{\matlabtextA $3.4$}%
\psfrag{009}[rc][rc]{\matlabtextA $3.8$}%
\psfrag{010}[rc][rc]{\matlabtextA $3.8$}%
%
%% </ytick>

==> gfx/power_time02.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA Idle}%
\psfrag{012}[cl][cl]{\matlabtextA Decodingaa}%
\psfrag{013}[bc][bc]{\matlabtextA Power}%
\psfrag{014}[tc][tc]{\matlabtextA Time}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $30$}%
\psfrag{001}[ct][ct]{\matlabtextA $40$}%
\psfrag{002}[ct][ct]{\matlabtextA $50$}%
\psfrag{003}[ct][ct]{\matlabtextA $60$}%
\psfrag{004}[ct][ct]{\matlabtextA $70$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $2.2$}%
\psfrag{006}[rc][rc]{\matlabtextA $2.6$}%
\psfrag{007}[rc][rc]{\matlabtextA $3$}%
\psfrag{008}[rc][rc]{\matlabtextA $3.4$}%
\psfrag{009}[rc][rc]{\matlabtextA $3.8$}%
\psfrag{010}[rc][rc]{\matlabtextA $3.8$}%
%
%% </ytick>

==> gfx/time_energy_HMRL1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{013}[cl][cl]{\matlabtextA data2}%
\psfrag{014}[cl][cl]{\matlabtextA Measuremenaaaaa}%
\psfrag{015}[bc][bc]{\matlabtextA Energy}%
\psfrag{016}[tc][tc]{\matlabtextA Time}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $20$}%
\psfrag{002}[ct][ct]{\matlabtextA $40$}%
\psfrag{003}[ct][ct]{\matlabtextA $60$}%
\psfrag{004}[ct][ct]{\matlabtextA $80$}%
\psfrag{005}[ct][ct]{\matlabtextA $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $10$}%
\psfrag{008}[rc][rc]{\matlabtextA $20$}%
\psfrag{009}[rc][rc]{\matlabtextA $30$}%
\psfrag{010}[rc][rc]{\matlabtextA $40$}%
\psfrag{011}[rc][rc]{\matlabtextA $50$}%
\psfrag{012}[rc][rc]{\matlabtextA $60$}%
%
%% </ytick>
